New computer-based search strategies for extreme functions of the Gomory--Johnson infinite group problem

We describe new computer-based search strategies for extreme functions for the Gomory--Johnson infinite group problem. They lead to the discovery of new extreme functions, whose existence settles several open questions.

==> Makefile <==
LATEX=latex
PDFLATEX=pdflatex
FIG2DEV=fig2dev
BIBTEX=bibtex

FIGURESDIRPREFIX=

MAINTEXFILE=mip-notes

all: $(MAINTEXFILE).pdf

%.pstex_t: %.fig #Makefile
	$(FIG2DEV) -L pstex_t -p $*.pstex $< $@

%.pstex: %.fig #Makefile
	$(FIG2DEV) -L pstex $< $@

%.pdftex_t: %.fig #Makefile
	$(FIG2DEV) -L pdftex_t -p $*.pdf $< $@

%.pdf: %.fig #Makefile
	$(FIG2DEV) -L pdftex $< $@

MIP_GRAPHICS_SOURCES=

MIP_GENERATED_GRAPHICS=$(MIP_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.pdftex_t) $(MIP_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.pdf) 

#$(MIP_GRAPHICS_SOURCES:%.fig=%.pstex_t) $(MIP_GRAPHICS_SOURCES:%.fig=%.pstex)

MIP_SOURCES=Makefile $(MAINTEXFILE).tex $(MIP_GRAPHICS_SOURCES:%.fig=$(FIGURESDIRPREFIX)%.fig) \
	sage-commands.tex 										\
	sage-commands-mip-notes.tex									\
	best-dim-threshold-table.tex									\
	denominators-table-figure.tex									\
	determinant-q11.tex										\
	vertex-enumeration-with-prep-table.tex								\
	vertex-enumeration-without-prep-table.tex

MIP_STYLES = bhk-style.tex

MIP_GRAPHICS=$(MIP_GENERATED_GRAPHICS)			\
	fulldim_covers_5slope_q22_1-2d_diagram.pdf	\
	fulldim_covers_5slope_q22_1-plot.pdf		\
	fulldim_covers_5slope_q22_2-2d_diagram.pdf	\
	fulldim_covers_5slope_q22_2-plot.pdf		\
	fulldim_covers_5slope_q22_3-2d_diagram.pdf	\
	fulldim_covers_5slope_q22_3-plot.pdf		\
	fulldim_covers_5slope_q22_4-2d_diagram.pdf	\
	fulldim_covers_5slope_q22_4-plot.pdf		\
	fulldim_covers_5slope_q22_5-2d_diagram.pdf	\
	fulldim_covers_5slope_q22_5-plot.pdf		\
	fulldim_covers_5slope_q22_6-2d_diagram.pdf	\
	fulldim_covers_5slope_q22_6-plot.pdf		\
	fulldim_covers_6slope_q25_1-2d_diagram.pdf	\
	fulldim_covers_6slope_q25_1-plot.pdf		\
	fulldim_covers_6slope_q26_1-2d_diagram.pdf	\
	fulldim_covers_6slope_q26_1-plot.pdf		\
	gj2s_interpolation.pdf				\
	gj2s_restriction.pdf				\
	gmic_interpolation.pdf				\
	gmic_restriction.pdf				\
	kzh_28_slope.pdf				\
	kzh_2q_example_1-2d_diagram.pdf			\
	kzh_2q_example_1-plot.pdf			\
	kzh_2q_move.pdf					\
	kzh_5_slope_fulldim_1-2d_diagram.pdf		\
	kzh_5_slope_fulldim_1.pdf			\
	kzh_10_slope_1-2d_diagram.pdf			\
	not_extreme_1-2d_diagram.pdf			\
	percentage_of_extreme.pdf			\
	q_v_grid.pdf					\
	scatterplotdenominator.pdf			\
	pattern_s6_q58.pdf				\
	pattern_s10_q166.pdf				\
	pattern_step0.pdf				\
	pattern_step1.pdf				\
	pattern_stept.pdf				\
	pattern_stepr1.pdf				\
	vertex_enumeration_time.pdf			\
	mean_time_exttest.pdf				\
	partial_painting_tree.pdf

BIB=../../bib/MLFCB_bib.bib

.PHONY: figures

figures: $(MIP_GRAPHICS) 

$(MAINTEXFILE).pdf: $(MAINTEXFILE).tex $(MIP_GRAPHICS) $(BIB)
	$(PDFLATEX) -halt-on-error "$<"
	$(BIBTEX) $(MAINTEXFILE)
	$(PDFLATEX) -halt-on-error "$<"
	$(PDFLATEX) -halt-on-error "$<"

MIP_SOURCES_AND_MORE=$(MIP_SOURCES) $(MIP_GRAPHICS) $(MIP_STYLES)

.PHONY: arxiv
arxiv:
	COPYFILE_DISABLE=true tar -cf $(CURDIR)/$(MAINTEXFILE).tar	\
		$(MAINTEXFILE).bbl					\
		$(MIP_SOURCES)					\
		$(MIP_GRAPHICS)					\
		$(MIP_STYLES)
	rm -f $(MAINTEXFILE).tar.gz
	gzip $(MAINTEXFILE).tar

